Trading Throughput for Freshness: Freshness-Aware Traffic Engineering and In-Network Freshness Control

In addition to traditional concerns such as throughput and latency, freshness is becoming increasingly important. To stay fresh, applications stream status updates among their components. Existing studies propose the metric age of information (AoI) to gauge the freshness and design systems to achieve low AoI. Despite active research in this area, existing results are not applicable to general wired networks for two reasons. First, they focus on wireless settings where AoI is mostly affected by interference and collision while queueing is more dominant in wired settings. Second, the legacy drop-adverse flows are not taken into account in the literature. Scheduling mixed flows with distinct performance objective is not yet addressed. In this paper, we study wired networks shared by two classes of flows, aiming for high throughput and low AoI respectively, and achieve a good trade-off between their throughput and AoI. Our approach to the problem consists of two layers: freshness-aware traffic engineering (FATE) and in-network freshness control (IFC). FATE derives sending rate/update frequency for flows via optimization, and its solution is then enforced by IFC through efficient scheduling mechanisms at each outport of in-network nodes. We also present efficient Linux implementation of IFC and demonstrate the effectiveness of FATE/IFC through extensive emulations. Our results show that it is possible to trade a little throughput (5 % lower) for much shorter AoI (49 to 71% shorter) compared to state-of-the-art traffic engineering.

==> analysis.tex <==
\section{Analysis}\label{sec:analysis}

In this section, we take an analytic approach to investigating the trade-offs in the IFC design.
We show that IFC, despite its simple design, yields an AoI not too far from the optimum, and derive properties of scheduler designs that are better than the one we propose, but show that there is a price to pay.
We defer the proofs of the theorems and the discussions on how to set the AoI ratio to achieve the optimal trade-off between throughput and AoI to Appendices.

\paragraph{Model and Notation}
We model the system as a single-link channel with capacity $C$, as illustrated in \fig{analysis_notation}. An AoI flow of inter-arrival time $T_i$ is queued at the AoI queue, which is governed by \IFIL. A scheduler, as described in \sec{design}, allows the AoI queue to send with the minimum output period $T_o$. Once the AoI queue is scheduled to send, an AoI packet is dequeued. The node serializes the update with transmission delay $d_t$ and sends it through the link with propagation delay $d_p$. Note that the transmission delay $d_t$ applies only to AoI packets and it is usually proportional to the size of the packet. Here, we simply model it as a constant. Finally, we assume the LDA flow can always fill the spare link bandwidth in between AoI updates.

\begin{figure}
\centering
\includegraphics{analysis_notation}
\vspace*{-0.5\baselineskip}
\caption{For analysis, we model the network as a link with capacity $C$ and propagation delay $d_p$.
We denote the inter-arrival time of the AoI flow by $T_i$, the minimum output period by $T_o$, and the transmission delay by $d_t$. Modeling LDA flows as fluid, we assume that LDA traffic can fully occupy the spare link bandwidth.}
\label{fig:analysis_notation}
\end{figure}

\subsection{\IFIL: Simple yet Effective}\label{sec:analysis-suboptimality}

IFC uses \IFIL to schedule the AoI queue.  \IFIL is simple to implement and its single flow version, \LIFOW, has been shown 
%to be
effective for Poisson/Bernoulli sources \cite{costa2014age, pappas2015age}. However, 
%it is also known that 
\IFIL can also perform quite badly under other arrival processes.
For example, consider a pulse train input with inter-arrival time $T_i = 1$~ns and a server that takes time $d_t$ to process each packet. Clearly, if $d_t \leq T_i$, every packet will arrive at an idle link and begin transmission immediately.
Suppose $d_t = 1.9$~ns. The second packet will arrive while the first is still being transmitted, and it will incur an additional age of $d_t - T_i = 0.9$~ns while it waits for the link to become available. Under \IFIL policy, the resulting AoI is $3.74$~ns.  Not only is this suboptimal, but a better policy is to simply have the link wait for an additional $0.1$~ns before transmitting queued packets. Doing so reduces the AoI to $2.9$~ns.\footnote{This waiting policy is also noted and discussed in \cite{sun2017update} for ``generate-at-will'' sources.}

Although this shows \IFIL can be suboptimal for pulse trains, it leaves open the question of just how suboptimal it is.
In the following theorem, we show that \IFIL only has a small constant factor loss compared to the optimum, even in the worst case of pulse trains. Given the simplicity of \IFIL, we argue that this provides good justification for the use of it in IFC.

\begin{theorem}\label{thm:LIFOW_bound}
Consider an AoI pulse train of inter-arrival time $T_i$ queued at the source going through a link. The AoI governed by \IFIL is at most $\frac{T_i}{2}$ more than the AoI governed by the optimal policy.
\end{theorem}


\subsection{Setting the AoI Ratio}\label{sec:analysis-setting-gamma}
\def\maxThr{M^{\rm thr}}
\def\minAoI{m^{\rm AoI}}

A key parameter for the design of IFC is the AoI ratio $\gamma$.
Every $\gamma$ value corresponds to a point on the trade-off curve, and so choosing $\gamma$ is crucial to balancing throughput and AoI. Recall that the ``closer'' a point on the trade-off curve is to the origin, the better the performance is. To define closeness to the origin, we need a framework to describe the desired trade-off. Formally, we propose to maximize the following objective
\begin{align}\label{eqn:optimal_gamma_condition_1}
\frac{\rm throughput}{\maxThr} - \lambda \ \frac{\rm AoI}{\minAoI}
\end{align}
where $\lambda \geq 0$ is a constant representing the trade-off factor. The throughput and AoI are normalized by the maximum possible throughput $\maxThr$ and the minimum possible AoI $\minAoI$, respectively.\footnote{By definition, $\maxThr$ is the capacity of the output link $C$, and $\minAoI = \frac{d_t}{2}$.} We maximize the objective \eqn{optimal_gamma_condition_1} by differentiating \eqn{optimal_gamma_condition_1} and setting it equal to 0, which gives
\begin{align}
\frac{\partial \rm throughput}{\partial \gamma} = \frac{\lambda \maxThr}{\minAoI} \frac{\partial \rm AoI}{\partial \gamma}.
\label{eqn:optimal_gamma_condition}
\end{align}

Using this equation, we derive the optimal $\gamma$ for both TDM and SDM in the following.

\paragraph{TDM} To derive the optimal $\gamma$ we take the time frame to be $T_f$ and suppose that in each AoI interval, at least one AoI packet is sent (i.e., $T_f \geq T_i$). After some calculation, the throughput and the AoI under TDM can be derived as
\begin{align*}
{\rm throughput} =&\ C \( \(1 - \frac{d_t}{T_i} \gamma \) - \( 1 - \frac{d_t}{T_i} \) \frac{d_t}{T_f}  \), \\
{\rm AoI} =&\
\frac{((1-\gamma)T_f+d_t)^2}{2 T_f} + \frac{T_i}{2} + d_t + d_p.
\end{align*}
By \eqn{optimal_gamma_condition}, the optimal $\gamma$ for TDM is then given by
\begin{align*}
\gamma =&\ 1 + \frac{d_t}{T_f} - \frac{d_t^2}{2 \lambda T_f T_i}.
\end{align*}

\paragraph{SDM}
Similarly to the case of TDM, we can compute the throughput and AoI under SDM:
\begin{align*}
{\rm throughput} =&\ C (1-\gamma), \\
{\rm AoI} =&\ \frac{1}{2}\(\frac{d_t}{\gamma} + T_i\) + d_{t} + d_p.
\end{align*}
Then, using \eqn{optimal_gamma_condition}, the optimal $\gamma$ for SDM is
\begin{align*}
\gamma = \sqrt{\lambda}.
\end{align*}

\begin{figure}
\includegraphics{analysis_setting_aoi_ratio}
\caption{The optimal AoI ratio $\gamma$ as a function of the trade-off factor $\lambda$. Given the same $\gamma$, SDM achieves optimal performance for larger $\lambda$, which emphasizes short AoI more than TDM.}
\label{fig:analysis_setting_aoi_ratio}
\end{figure}

To illustrate the contrast between $\gamma$ under TDM and SDM, we use the settings in \fig{scheduler_comparison_setup} and plot the optimal $\gamma$ under different $\lambda$ in \fig{analysis_setting_aoi_ratio}. To achieve the optimal trade-off under a given $\lambda$, TDM requires a significantly larger $\gamma$ than SDM. This means that, given the same $\gamma$, SDM would emphasize short AoI more than TDM.


\subsection{Price to Pay for Better Schedulers}\label{sec:analysis-transition-point-effect}

\fig{tradeoff_throughput_aoi} shows that neither TDM nor SDM uniformly outperforms the other.
Thus, a natural question is whether it is possible to design a scheduler that outperforms both TDM and SDM, taking the best from each. Below we derive a property that must be true of any scheduler that is better than both TDM and SDM, then illustrate why one may not want to use such a design.

\begin{theorem}\label{thm:better-scheduler}
Consider the system in \fig{analysis_notation}. If a scheduling algorithm outperforms TDM under any given $d_p$ and $T_i > 2 d_t$, it must have $T_o = 0$ or it is not work conserving for the AoI queue.
\end{theorem}

\thm{better-scheduler} highlights that if a scheduler outperforms both TDM and SDM, it must impose zero
gap between the service of two consecutive AoI packets, or it should be able to wait even when the AoI queue is not empty.
We remark that \thm{better-scheduler} does not require the scheduler to keep serving the AoI queue. Rather, it says that the scheduler must either occasionally allow intermittent bursts of AoI packets or deliberately put AoI packets on hold. Of course, such bursts come at the direct expense of the LDA packets and so these bursts cannot be too frequent. Likewise, the waiting policy is nontrivial to derive. This highlights the drawbacks of such a design. To enable intermittent bursts of AoI packets or delayed output, the scheduler needs an additional state to keep track of the number of output AoI packets. The introduction of the additional state complicates the scheduler design and slows down the processing of each packet. Further, setting the frequency of the AoI bursts/halt period so as to balance the AoI and LDA traffic depends on fine-grained details of the workload, which adds additional complexity and overhead.  In contrast, by using either TDM or SDM, as appropriate for the networks, we have a significantly lighter implementation and operation overhead while performing nearly optimally in practice.


